PureEBM: Universal Poison Purification via Mid-Run Dynamics of Energy-Based Models

Data poisoning attacks pose a significant threat to the integrity of machine learning models by leading to misclassification of target distribution data by injecting adversarial examples during training. Existing state-of-the-art (SoTA) defense methods suffer from limitations, such as significantly reduced generalization performance and significant overhead during training, making them impractical or limited for real-world applications. In response to this challenge, we introduce a universal data purification method that defends naturally trained classifiers from malicious white-, gray-, and black-box image poisons by applying a universal stochastic preprocessing step $\Psi_{T}(x)$, realized by iterative Langevin sampling of a convergent Energy Based Model (EBM) initialized with an image $x.$ Mid-run dynamics of $\Psi_{T}(x)$ purify poison information with minimal impact on features important to the generalization of a classifier network. We show that EBMs remain universal purifiers, even in the presence of poisoned EBM training data, and achieve SoTA defense on leading triggered and triggerless poisons. This work is a subset of a larger framework introduced in \pgen with a more detailed focus on EBM purification and poison defense.

==> EBM/Algos/train_clf.tex <==
\begin{algorithmic}
\REQUIRE Train dataset $X$, Model $F_\phi$, LR $\eta_{opt}$ %, Epochs $T$ 
\ENSURE Pre-process dataset via MCMC: $\Tilde{X}\gets\Psi_{T}(X)$
\STATE Initialize weights $\phi_1$ for Classifier $F$
\WHILE{$\phi_i$ not converged}
    \STATE $i \gets i + 1$\\ 
    \FOR{$\Tilde{x} \in \Tilde{X}$}
        \STATE Calculate the Grads and Update Params
        \STATE $\mathfrak{g}_i \gets \nabla_{\phi}F_{\phi_{i-1}}(\Tilde{x}_i)$
        \STATE $\phi_i \gets \phi_{t-1} - \eta_{opt} \mathfrak{g}_t$ 
    \ENDFOR
\ENDWHILE
\end{algorithmic}
% \begin{algorithmic}
   % \REQUIRE {Train dataset $X$, Model $f_\theta$, LR $\eta_{opt}$, $\lambda$, small number $T$}
   %  \FOR{$i = 1 \to T$}
   %      \STATE $\theta^i = \theta^{i-1} - \eta \nabla_{\theta} L(\theta^{i-1}, X)$ \Comment{Train the model for a few epochs}
   %  \ENDFOR
% \end{algorithmic}




==> EBM/Algos/train_ebm.tex <==
\begin{algorithmic}
\REQUIRE ConvNet potential $U(x; \theta)$, images $x^+_i \in  \mathcal{X} or (\mathcal{X} \setminus \mathcal{P}_{all})$, Langevin steps $K=100$, temp $\tau=1e-4$, image bank $\{ Y \}_{i=1}^{1250}$
\ENSURE Weights $\theta_{J+1}$ for $U(x ; \theta)$
\STATE Initialize image bank $\{ Y \}_{i=1}^s$ with $s=1250$ images
\FOR{$j$ in iters}
    \STATE Draw batch $\{x_{(i)}^+\}_{i=1}^m$; initial negatives $\{ Y_i^{(0)} \}_{i=1}^m$ from $\{ Y \}$
    \STATE Update $\{ Y_i^{(0)} \}$ using Langevin dynamics:
        \[ Y^{(k)}_i = Y^{(k-1)}_i - \frac{\tau^2}{2} \nabla_y U(Y^{(k-1)}_i ; \theta_j) + \tau Z_{i, k} \]
    \STATE Update image bank $\{ Y_i^{(K)} \}_{i=1}^m$; weights $\theta_{j+1}$ using:
        \[ \Delta \theta_j= \nabla_\theta \left( \frac{1}{n} \sum_{i=1}^n U(X^+_i ; \theta_j) - \frac{1}{m}\sum_{i=1}^m U(X_i^-; \theta_j) \right) \]
\ENDFOR
\end{algorithmic}

==> EBM/Tables/models_and_datasets.tex <==
\begin{tabular}{@{}lllll@{}}
\toprule
\multicolumn{5}{c}{\textbf{CINIC-10 Narcissus - 1\% From-Scratch (200 Epochs)}}                                                                                                                                                                                                                                                                                                                           \\ \midrule
                                             & \multicolumn{1}{c}{\begin{tabular}[c]{@{}c@{}}Avg Poison \\ Success (\%) ↓\end{tabular}} & \multicolumn{1}{c}{\begin{tabular}[c]{@{}c@{}}Avg Natural\\  Accuracy (\%) ↑\end{tabular}} & \multicolumn{1}{c}{\begin{tabular}[c]{@{}c@{}}Max Poison \\ Success (\%) ↓\end{tabular}} & \multicolumn{1}{c}{\begin{tabular}[c]{@{}c@{}}CIFAR-10\\ Accuracy (\%) ↑\end{tabular}} \\ \midrule
\multicolumn{1}{l|}{None}                    & 62.06$_{0.21}$                                                                      & 86.32$_{0.10}$                                                                          & 90.79                                                                           & 94.22$_{0.16}$                                                                      \\
\multicolumn{1}{l|}{\epic}    & 49.50$_{0.27}$                                                                        & 81.91$_{0.08}$                                                                          & 91.35                                                                           & 91.10$_{0.21}$                                                                      \\
\multicolumn{1}{l|}{\friends} & 11.17$_{0.25}$                                                                        & 77.53$_{0.60}$                                                                          & 82.21                                                                           & 88.27$_{0.68}$                                                                      \\
\multicolumn{1}{l|}{\pebm}    & \textbf{7.73$_{0.08}$}                                                                & \textbf{82.37$_{0.14}$}                                                               & \textbf{29.48}                                                                  & \textbf{91.98$_{0.16}$}                                                           \\ \bottomrule
\toprule
                                        \multicolumn{5}{c}{\textbf{From Scratch NS-1\% (200 epochs)}}                                                                                                                                                                                                                     \\ \midrule
\textbf{}                                              & \multicolumn{2}{c}{\textbf{MobileNetV2}}                                                                                                   & \multicolumn{2}{c}{\textbf{DenseNet121}}                                                                                             \\ \cmidrule(lr){2-3}\cmidrule(lr){4-5} 
\textbf{}                                              & \begin{tabular}[c]{@{}c@{}}Avg Poison \\ Success  (\%) ↓\end{tabular} & \begin{tabular}[c]{@{}c@{}}Avg Natural \\ Accuracy (\%) ↑\end{tabular}       & \begin{tabular}[c]{@{}c@{}}Avg Poison \\ Success  (\%) ↓\end{tabular} & \begin{tabular}[c]{@{}c@{}}Avg Natural \\ Accuracy (\%) ↑\end{tabular} \\ \midrule
\multicolumn{1}{l|}{None}                              & 32.70$_{0.25}$                                                     & 93.92$_{0.13}$                                             & 46.52$_{32.2}$                                                                        & 95.33$_{0.1}$                                                                                                             \\
\multicolumn{1}{l|}{\epic}              & 22.35$_{0.24}$                                                     & 78.16$_{9.93}$                                                            & 32.60$_{29.4}$                                                                        & 85.12$_{2.4}$                                                         \\
\multicolumn{1}{l|}{\friends}           & 2.00$_{0.01}$                                                      & 88.82$_{0.57}$                                                             & 8.60$_{21.2}$                                                                         & 91.55$_{0.3}$                                                           \\
\multicolumn{1}{l|}{\textbf{\pebm}}     & \textbf{1.64$_{0.01}$}                                             & \textbf{91.75$_{0.13}$}                                                   & \textbf{1.42$_{0.7}$}                                                                 & \textbf{93.48$_{0.1}$}                                                         \\ \midrule
                                      \multicolumn{5}{c}{\textbf{Linear Transfer  WhiteBox BP-10\%}}                                                                                                                                                                                                                    \\ \midrule
                                                       & \multicolumn{2}{c}{\textbf{MobileNetV2}}                                                                                                   & \multicolumn{2}{c}{\textbf{DenseNet121}}                                                                                             \\ \cmidrule(lr){2-3}\cmidrule(lr){4-5} 
                                                       & \begin{tabular}[c]{@{}c@{}}Poison \\ Success (\%) ↓\end{tabular}      & \begin{tabular}[c]{@{}c@{}}Avg Natural \\ Accuracy (\%) ↑\end{tabular}       & \begin{tabular}[c]{@{}c@{}}Poison \\ Success (\%) ↓\end{tabular}      & \begin{tabular}[c]{@{}c@{}}Avg Natural \\ Accuracy (\%) ↑\end{tabular} \\ \midrule
\multicolumn{1}{l|}{None}                              & 81.25                                                          & 73.27$_{0.97}$                                                            & 73.47                                                          & 82.13$_{1.62}$                                                      \\
\multicolumn{1}{l|}{\epic}              & 56.25                                                          & 54.47$_{5.57}$                                                            & 66.67                                                          & 70.20$_{10.15}$                                                     \\
\multicolumn{1}{l|}{\friends}           & 41.67                                                          & 68.86$_{1.50}$                                                            & 60.42                                                          & 80.22$_{1.90}$                                                      \\
\multicolumn{1}{l|}{\textbf{\pebm}}     & \textbf{0.00}                                                  & \textbf{78.57$_{1.37}$}                                                   & \textbf{0.00}                                                  & \textbf{89.29$_{0.94}$}                                             \\ \midrule
      \multicolumn{5}{c}{\textbf{Hyperlight Bench CIFAR-10 NS-1\% (10 Epochs)}}                                                                                                                                                                                                         \\ \midrule
                                                       & \begin{tabular}[c]{@{}c@{}}Avg Poison \\ Success (\%) ↓\end{tabular} & \begin{tabular}[c]{@{}c@{}}Avg Natural \\ Accuracy (\%) ↑\end{tabular} & \begin{tabular}[c]{@{}c@{}}Max Poison\\ Success (\%) ↓\end{tabular}   & \begin{tabular}[c]{@{}c@{}}Train Time (s) \\ (Epoch Time)\end{tabular} \\ \midrule
\multicolumn{1}{l|}{None}                              & 76.39$_{16.35}$                                                  & 93.95$_{0.10}$                                                          & 95.69                                                            & 6.81$_{0.62}$ (0.68)                                                                  \\
\multicolumn{1}{l|}{\epic}              & 10.58$_{18.35}$                                                  & 24.88$_{6.04}$                                                          & 50.21                                                            & 612.43$_{30.16}$ (61.24)                                                              \\
\multicolumn{1}{l|}{\friends}           & 11.35$_{18.45}$                                                  & 87.03$_{1.52}$	                                                          & 56.65	                                                            & 427.50$_{0.50}$ (42.75)                                                                  \\
\multicolumn{1}{l|}{\textbf{\pebm-25}}  & 10.59$_{26.04}$                                                  & 92.75$_{0.13}$                                                          & 84.60                                                            & 54.70$_{0.48}$ (0.65)                                                                 \\
\multicolumn{1}{l|}{\textbf{\pebm-50}}  & \textbf{2.16$_{1.22}$}                                           & \textbf{92.38$_{0.17}$}                                                 & \textbf{3.74}                                                    & 92.89$_{0.48}$ (0.64)                                                                 \\
\multicolumn{1}{l|}{\textbf{\pebm-100}} & \textbf{1.89$_{1.06}$}                                           & \textbf{91.94$_{0.14}$}                                                 & \textbf{3.47}                                                    & 168.69$_{0.46}$ (0.64)                                                                \\
\multicolumn{1}{l|}{\textbf{\pebm-150}} & \textbf{1.93$_{1.15}$}                                           & \textbf{91.46$_{0.17}$}                                                 & \textbf{4.14}                                                    & \multicolumn{1}{c}{244.72$_{0.47}$ (0.64)}                                            \\
\multicolumn{1}{l|}{\textbf{\pebm-300}} & \textbf{1.68$_{0.82}$}                                           & \textbf{90.55$_{0.21}$}                                                 & \textbf{2.89}                                                    & \multicolumn{1}{c}{478.29$_{0.47}$ (0.64)}                                            \\ \bottomrule
\vspace{-7mm}
\end{tabular}


==> EBM/Tables/natural_ebms.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{booktabs}
\begin{tabular}{@{}lccc@{}}
\toprule
\multicolumn{4}{c}{\textbf{From Scratch GM-1\% (200 Epochs)}}                                                                                                                                                                              \\ \midrule
                                          & \begin{tabular}[c]{@{}c@{}}Poison \\ Success $\downarrow$\end{tabular}     & \multicolumn{2}{c}{\begin{tabular}[c]{@{}c@{}}Avg Natural \\ Accuracy $\uparrow$\end{tabular}}                                            \\ \midrule
\multicolumn{1}{l|}{\pebm} & \textbf{0.00\%}                                               & \multicolumn{2}{c}{\textbf{92.26\%±0.22}}                                                                                      \\ \cmidrule(r){1-1}
\multicolumn{1}{l|}{\pebm$_{cinic10}$} & \textbf{0.00\%}                                               & \multicolumn{2}{c}{\textbf{92.99\%±0.22}}                                                                                      \\
\multicolumn{1}{l|}{\pebm$_{imagenet}$} & 1.00\%                                                        & \multicolumn{2}{c}{\textbf{92.98\%±0.18}}                                                                                      \\ \midrule
\multicolumn{4}{c}{\textbf{From Scratch NS-1\% (200 Epochs)}}                                                                                                                                                                              \\ \midrule
                                          & \begin{tabular}[c]{@{}c@{}}Avg Poison \\ Success $\downarrow$\end{tabular} & \begin{tabular}[c]{@{}c@{}}Avg Natural \\ Accuracy $\uparrow$\end{tabular} & \begin{tabular}[c]{@{}c@{}}Max Poison\\ Success $\downarrow$\end{tabular} \\ \midrule
\multicolumn{1}{l|}{\pebm} & \multicolumn{1}{l}{\textbf{1.27\%±0.01}}                      & \multicolumn{1}{l}{\textbf{92.91\%±0.17}}                       & \textbf{2.16\%}                                              \\
\multicolumn{1}{l|}{\pebm-p} & \multicolumn{1}{l}{\textbf{1.38\%±0.01}}                      & \multicolumn{1}{l}{\textbf{92.70\%±0.21}}                       & \textbf{2.78\%}                                              \\ \cmidrule(r){1-1}
\multicolumn{1}{l|}{\pebm$_{cinic10}$} & \multicolumn{1}{r}{\textbf{1.43\%±0.01}}                      & \multicolumn{1}{r}{\textbf{92.90\%±0.19}}                       & \textbf{3.06\%}                                              \\
\multicolumn{1}{l|}{\pebm$_{imagenet}$} & \multicolumn{1}{r}{\textbf{1.39\%±0.01}}                      & \multicolumn{1}{r}{\textbf{92.92\%±0.16}}                       & \textbf{2.50\%}                                              \\
\multicolumn{1}{l|}{\pebm-p$_{cinic10}$} & \multicolumn{1}{r}{\textbf{1.64\%±0.01}}                      & \multicolumn{1}{r}{\textbf{92.86\%±0.20}}                       & \textbf{4.34\%}                                              \\ \midrule
\multicolumn{4}{c}{\textbf{Transfer Linear BP-10\% (BlackBox)}}     \\ \midrule
                                          & \begin{tabular}[c]{@{}c@{}}Poison \\ Success $\downarrow$\end{tabular}     & \multicolumn{2}{c}{\begin{tabular}[c]{@{}c@{}}Avg Natural \\ Accuracy $\uparrow$\end{tabular}}                                            \\ \midrule
\multicolumn{1}{l|}{\pebm} & \textbf{0.00\%}                                               & \multicolumn{2}{c}{\textbf{92.89\%±0.19}}                                                                                      \\ \cmidrule(r){1-1}
\multicolumn{1}{l|}{\pebm$_{cinic10}$} & \textbf{0.00\%}                                               & \multicolumn{2}{c}{\textbf{92.82\%±0.15}}                                                                                      \\
\multicolumn{1}{l|}{\pebm$_{imagenet}$} & \textbf{0.00\%}                                               & \multicolumn{2}{c}{\textbf{92.38\%±0.29}}                                                                                     
\end{tabular}


==> EBM/method_long.tex <==
\subsection{Methods Long}
EBMs are trained by performing a forward pass and MCMC sampling, which is a distinct process from score-based models that do not use sampling during training. EBM is a Gibbs-Boltzmann density \citep{xie2016theory}.  A deep EBM has the form:

\begin{align}
p(x; \theta)=\frac{1}{Z(\theta)} \exp\{-\mathcal{G}_{\theta}(x)\} \label{eqn:ebm}
\end{align}

where $x \in R^D$ is an image signal. The energy $\mathcal{G}_{\theta}(x)$ is a ConvNet with weights $\theta$, a scalar output, and $Z(\theta) = \int_{\mathcal{X}} \exp{[-\mathcal{G}_{\theta}(x)]}\,dx$ is the intractable normalizing constant, which is never used because the energy $\mathcal{G}_{\theta}(x)$ provides sufficient information in Markov Chain Monte Carlo (MCMC) sampling in unsupervised Maximum Likelihood Estimation (MLE) learning. The goal of MLE learning is to find $\theta \in \Theta$ from a data distribution $q(x)$ such that the parametric model $p(x;\theta) \approx q(x)$ by minimizing the expected negative log-likelihood, given i.i.d samples.:


\begin{align}
L(\theta) = E_q[-\mathrm{log} p(x;\theta)]
\label{eqn:KL}
\end{align}


MLE learning uses the objective function by minimizing Kullback-Leibler (KL) divergence $\argmin_{\theta} D_{KL} (q(x) || p(x;\theta))$:

\begin{equation}
\begin{aligned}
\argmin_{\theta} L(\theta) &= \argmin_{\theta} D_{KL} (q(x) || p(x;\theta))\\
                           &= \argmin_{\theta} E_q [\log \frac{q}{p_{\theta}}]\\
                           &= \argmin_{\theta} \int q \log \frac{q}{p_{\theta}} \,dx \\
                           &= \argmin_{\theta} ( \int q \log q \,dx - \int q \log p_{\theta} \,dx )\\
                           &= \argmin_{\theta} (\underbrace{E_q \log q }_\text{-entropy} \underbrace{-E_q \log p_{\theta}}_{L(\theta)} ) \\
                           &= \argmin_{\theta} ( -H(q) +  H(q,p_{\theta}) ) 
\label{eqn:ebmKL}
\end{aligned}
\end{equation}

Gradient descent is used for minimizing the objective function $L(\theta)$. Since only the cross entropy term contains $\theta$. It's also equivalent to minimize the cross entropy $H(q,p_{\theta}) = -E_q \log p_{\theta} = - E_q \log \frac{1}{z(\theta)} \exp([-\mathcal{G}_{\theta}(x)])$. The derivative of the loss is:


\begin{align}
\nabla \mathcal{L}(\theta) &= \nabla \log z(\theta) + \nabla E_q [ \mathcal{G}_{\theta}(x) ] 
\label{eqn:ebmlearning}
\end{align}


where the $\nabla \log z(\theta) $ can be expressed as:

\begin{equation}
\begin{aligned}
\nabla \log z(\theta) &= \frac{1}{z(\theta)} \nabla z(\theta) \\
      &= \frac{1}{z(\theta)} \nabla \int \exp{[-\mathcal{G}_{\theta}(x)]} \,dx\\
      &= \frac{1}{z(\theta)} \int  \exp{[-\mathcal{G}_{\theta}(x)]}  \nabla [-\mathcal{G}_{\theta}(x)] \,dx\\
      &= \int \frac{1}{z(\theta)} \exp{[-\mathcal{G}_{\theta}(x)]} \nabla [-\mathcal{G}_{\theta}(x)] \,dx \\
      &= \int p_{\theta} \nabla [-\mathcal{G}_{\theta}(x)] \,dx \\
      &= - E_{p_{\theta}} [\nabla \mathcal{G}_{\theta}(x)] 
\label{eqn:logz}
\end{aligned}
\end{equation}

Thus, the gradient used to learn $\theta$ becomes:

\begin{equation}
\begin{aligned}
\nabla \mathcal{L}(\theta) &= \nabla  E_q [ \mathcal{G}_{\theta}(x) ]  - \nabla E_{p_{\theta}} [ \mathcal{G}_{\theta}(x) ] \\
      &\approx \frac{1}{n}\sum_{i=1}^n \nabla_\theta \mathcal{G}_{\theta}(X_i^+)-\frac{1}{m}\sum_{i=1}^{m} \nabla_\theta \mathcal{G}_{\theta}(X_i^-)
\label{eqn:ebmgrad}
\end{aligned}
\end{equation}


where the positive samples $\{x_i^+\}_{i=1}^n$ are a set of data samples and the negative samples $\{x_i^-\}_{i=1}^k$ are samples from the current model $p(x;\theta)$. In practice, the positive samples $\{x_i^+\}_{i=1}^n$ are a batch of training images and negative samples $\{x_i^-\}_{i=1}^k$ are obtained after T iterations of MCMC sampling.

To obtain the negative samples for a deep EBM, it is common to use MCMC sampling with the $T$ steps of Langevin Dynamics (LD) equation

\begin{align}
x_{\tau+1} = x_{\tau} - \Delta \tau \nabla_{x_{\tau}} \mathcal{G}_{\theta}(x_{\tau}) + \sqrt{2\Delta \tau} \epsilon_{\tau}  ,\label{eqn:langevin_apdx}
\end{align}

where $\epsilon$ is the step size and $Z_k \sim N(0, I^D)$. The Langevin trajectories are initialized from a set of states $\{X^-_{i, 0}\}_{i=1}^n$ obtained from a certain initialization strategy. The method of MCMC initialization determines many of the properties of the learned model.

\cite{nijkamp2019anatomy} presented the anatomy of MCMC-Based ML Learning of EBMs, which introduced two axes of ML learning. One axis is expansion or contraction, the other is convergence or Non-convergence. \cite{hinton2002poe} introduced Contrastive Divergence that initializes from the data $U(X_i^+;\theta)$. Persistent initialization is from negative samples $U(X_i^-;\theta)$ from a previous MCMC iteration. It can be from noise \citep{xie2016theory} or data \citep{tieleman2008training}. Cooperative learning generalizes the persistent chains by learning a generator \citep{xie_coop} in tandem with the energy.

EBMs can be small, flexible and fast to train. They can also be trained with large data sets and high-resolution images without memory issues compared to diffusion models. During the training process,  iterative MCMC sampling is used to obtain the negative samples from the learned distribution. The length of the MCMC samplings determines the different properties of EBMs \citep{hill2022ebm}. Short-run EBMs with a few hundred of steps are sufficient for high quality image synthesis \citep{nijkamp2019anatomy}. Mid-run EBMs with a few thousands of steps are proper for adversarial defense \citep{hill2021stochastic}. Long-run EBMs with 1 million or more steps are valid for density estimation \citep{nijkamp2019anatomy, hill2021stochastic}.

% 



\begin{algorithm}[ht]
\caption{ML with SGD for Convergent Learning of EBM (\ref{eqn:ebm})}
\begin{algorithmic}
\REQUIRE ConvNet potential $f_{\theta}(x)$, number of training steps $J=150000$, initial weight $\theta_1$, training images $\{x^+_i \}_{i=1}^{N_\textrm{data}}$, data perturbation $\tau_\text{data}=0.02$, step size $\tau=0.01$, Langevin steps $K=100$, SGD learning rate $\gamma_\text{SGD}=0.00005$.
\ENSURE Weights $\theta_{J+1}$ for energy $f_{\theta}(x )$.\\
\STATE
\STATE Set optimizer $g \leftarrow \text{SGD}(\gamma_\text{SGD})$. Initialize persistent image bank as $N_\text{data}$ uniform noise images.
\FOR{$j$=1:($J$+1)}
\begin{enumerate}
    \item Draw batch images $\{x_{(i)}^+\}_{i=1}^m$ from training set, where $(i)$ indicates a randomly selected index for sample $i$, and get samples $X_i^+ = x_{(i)} + \tau_\text{data} \epsilon_i$, where $\epsilon_{i} \sim \textrm{N}(0, I_D)$ i.i.d.
    
    \item Draw initial negative samples $\{ Y_i^{(0)} \}_{i=1}^m$ from persistent image bank.
    			Update $\{ Y_i^{(0)} \}_{i=1}^m$ with the Langevin equation 
    			\begin{align*}
    			Y^{(k)}_i = Y^{(k-1)}_i +  \Delta \tau \nabla_{Y_{\tau}} f_{\theta_j}(Y_i^{\tau-1}) 
       % U(Y^{(k-1)}_i ; \theta_j) 
       + \tau \epsilon_{i, k} ,
                % x_{\tau+1} = x_{\tau} + \Delta \tau \nabla_{x_{\tau}} f_{\theta}(x_{\tau}) + \sqrt{2\Delta \tau} \epsilon_{\tau}  
    			\end{align*}
    			 where $\epsilon_{i , k} \sim \textrm{N}(0, I_D)$ i.i.d., for $K$ steps to obtain samples $\{ X_i^- \}_{i=1}^m = \{ Y_i^{(K)} \}_{i=1}^m$. Update persistent image bank with images $\{ Y_i^{(K)} \}_{i=1}^m$.
    \item Update the weights by $\theta_{j+1} = \theta_{j} - g(\Delta \theta_j)$, where $g$ is the optimizer and 
    			\[
    			\Delta \theta_j= \frac{\partial}{\partial \theta} \left( \frac{1}{n} \sum_{i=1}^n f_{\theta_j}(X^+_i ) - \frac{1}{m}\sum_{i=1}^m f_{\theta_j}(X_i^-) \right)
    			\]
    			is the ML gradient approximation.
\end{enumerate}
\ENDFOR
\end{algorithmic}
\label{al:ml_learning}
\end{algorithm}

==> EBM/variable_defs.tex <==
% \section{To Be Removed}

% \subsection{Variable Definitions (main paper only)}

% \begin{itemize}
%     \item $\Psi(x)$: Stochastic transformation function applied to the input image $x$.
%     \item $x \in \mathbb{R}^D$: Input image or data sample
%     \item $y$: Image label
%     \item $\delta$ and $\rho$: Small adversarial perturbations injected into a fraction of training images. $\delta$ for dataset perturbations, $\rho$ for patch. 
%     \item $\alpha$: The fraction of train images that are poisoned.
%     \item $y^{adv}$: Target label/class for poison method
%     \item $\mathcal{D}$: Dataset of images and labels (test, train); has length $n$. 
%     \item $\mathcal{X}$: Images dataset (test, train)
%     \item $\Pi = \{ (x^\pi , y^\pi) \}$  The set of target image, label pairs
%     \item $F$: Classifier
%     \item $\mathcal{C}$: Set of allowable poisons
%     \item $\eta$: Learning rate
%     \item $\theta$ and $\phi$: Parameters or weights of a model, $\theta$ for EBM, $\phi$ for classifier.
%     % \item $\phi(x)$: 
%     \item $\xi$: Small value representing the magnitude of perturbation in adversarial attacks, often used in the context of crafting adversarial examples.
%     \item $\mathcal{G}(x)$: Energy function in an Energy-Based Model (EBM), where $x$ is the input and $\theta$ represents the parameters of the model.
%     \item $Z$: Partition function, normalizing constant in the context of EBMs.
%     \item $p_{\theta}(x)$: Learned probability distribution function parameterized by $\theta$ in the context of EBMs.
%     \item $L(\theta)$: Loss function with respect to the parameters $\theta$.
%     \item $\nabla L(\theta)$: Gradient of the loss function with respect to the parameters $\theta$.
%     \item $T$: Number of steps in MCMC chain
%     \item $\tau$: Current Step in MCMC chain
%     \item $\gamma$: A parameter, possibly related to the step size in Langevin dynamics or a noise parameter in stochastic processes.
%     \item $X(k)$: State of a system or a sample at step $k$ in Langevin dynamics.
%     \item $\epsilon$: Step size or learning rate parameter, particularly in the context of iterative update rules like Langevin dynamics.
% \end{itemize}

% Appendix

% \begin{itemize}
%     \item $\lambda$: Lyapunov exponent used in the context of chaos theory and dynamical systems.
% \end{itemize}

==> EPIC/proof.tex <==

\textbf{Polyak-Lojasiewicz (PL) condition}

A loss function $\mathcal{L}(w)$ is considered $\mu$ -PL on a set $\mathcal{S}$, if the following holds:
\begin{align}
    \frac{1}{2}\|\mathbf{g}\|^{2} \geq \mu\left(\mathcal{L}(w)-\mathcal{L}\left(w_{*}\right)\right), \forall w \in \mathcal{S}
    \label{eq:pl}
\end{align}
where $w_{*}$ is a global minimizer.
When additionally $\mathcal{L}\left(w_{*}\right) = 0$, 
the $\mu$-$\text{PL}$ condition is equivalent to the $\mu$-$\text{PL}^{*}$ condition 
\begin{align}
    \frac{1}{2}\|\mathbf{g}\|^{2} \geq \mu\mathcal{L}(w), \forall w \in \mathcal{S}.
\end{align}
For Lipschitz continuous $\mathbf{g}$ and $\mu$-PL$^*$ condition, gradient descent on the entire dataset yields
\begin{align}
    \mathcal{L}(w_{t+1}) - \mathcal{L}(w_t) \leq -\frac{\eta} {2}\|\mathbf{g}_t\|^2 \leq -\eta\mu \mathcal{L}(w_t),\label{eq:grad_rate}
\end{align}
and,

\begin{align}
    \mathcal{L}(w_{t})\leq(1-\eta\mu)^t \mathcal{L}(w_0),\label{eq:lip}
\end{align}
which was shown in \cite{liu2020toward}.
\begin{restatable}{theorem}{plrestate}
\label{thm:pl}
    Assume that the loss function $\Lc(w)$ is $\beta$-smooth, and $\mu$-PL$^*$ on a set $\mathcal{W}$, and $S$ is a weighted subset %of size $r$
    obtained by \alg that estimates the general descent direction by an error of at most $\varepsilon$, i.e., $\| \sum_{i\in V}\textbf{g}_{t,i}-\sum_{j\in S}\gamma_{t,j}\textbf{g}_{t,j}\|\leq\varepsilon$. 
    Then with learning rate $\eta$, gradient descent with update rule of Eq. \eqref{eq:gd_update} %with $m_t=\mathbf{g}$ and $v_t=1$
    applied to the subsets have the following convergence behavior at iteration $t$:
    Then for the iterates $\{w_0, \cdots, w_T\}$ generated by applying \alg to $S$ with stepsize $\eta$, we have 
\begin{align}    
    \Lc(w_{t}) \leq (1-\eta\mu)^{t} \Lc(w_0) + \frac{1}{2\mu}(\varepsilon^2+2\varepsilon \nabla_{\max}),
\end{align}
where  $\nabla_{\max}$ is an upper-bound on the norm of the gradients.
\end{restatable}


\begin{proof}    
    First to take care of some notation: 
    \begin{itemize}
        \item     We define $\mathbf{g}_t^S \triangleq \sum_{j\in S}\gamma_{t,j}\textbf{g}_{t,j}$ , where $S$ is some subset and $\sum_{j\in S}\gamma_{t,j} = 1$ where $\gamma_{t,i} \geq 0 \quad \forall t,i.$ 
        \item  We define $\mathbf{g}_t \triangleq \sum_{j\in V}\textbf{g}_{t,i}$ where $V$ is the full dataset. 
    \end{itemize}
    
    For the subset we have
    \begin{align}
        \Lc(w_{t+1}) - \Lc(w_t) 
        &\leq -\frac{\eta}{2}\|\mathbf{g}_t^S\|^2
        \label{eq:subset}
    \end{align}    
   
   We apply the reverse triangle inequality to $\| \mathbf{g}_t-\mathbf{g}_t^S\|\leq\varepsilon$ to get $\|\mathbf{g}_t \| \leq \|\mathbf{g}_t^S \| + \varepsilon$ which substituted in \eqref{eq:subset} yields
    \begin{align}
        &\leq -\frac{\eta}{2}(\|\mathbf{g}_t\|-\varepsilon)^2\\
        &= -\frac{\eta} {2}(\|\mathbf{g}_t\|^2+\varepsilon^2-2\varepsilon\|\mathbf{g}_t\|)\label{eq:pre_spectral_upper}\\
        &\leq - \frac{\eta} {2}(\|\mathbf{g}_t\|^2+\varepsilon^2-2\varepsilon \nabla_{\max})\\
        &\leq -\frac{\eta} {2}(2\mu \mathcal{L}(w_t)+\varepsilon^2-2\varepsilon \nabla_{\max}) \label{eq:pl_applied}
    \end{align}
    % Where we 
    where we can upper bound the norm of $\mathbf{g}_t$ in Eq. (\ref{eq:pre_spectral_upper}) by a constant $\nabla_{\max}$. And Eq. (\ref{eq:pl_applied}) follows from the $\mu$-PL condition from Eq. (\ref{eq:pl}). While the loss is very non-convex during the first part of training, it becomes nearly convex afterward \cite{fort2020deep}.  \epic~starts dropping points after a few epochs of training, where Lipschitzness, $\mu$-PL condition, and norm-bounded gradients are likely to hold. In Eq. \eqref{eq:lip}, LHS directly results from Lipschitzness \cite{boyd2004convex}.

    
    
    
    
    Hence,
    \begin{align}
        \mathcal{L}(w_{t+1}) \leq (1-{\eta\mu} ) \mathcal{L}(w_t) - \frac{\eta} {2}(\varepsilon^2-2\varepsilon \nabla_{\max})\label{eq:step1}
    \end{align}
    Applying \eqref{eq:step1} recursively
    \begin{align}
        \mathcal{L}(w_{t+1}) \leq (1-{\eta\mu} {})^{t+1} \mathcal{L}(w_0) - \frac{\eta}{2}(\varepsilon^2-2\varepsilon \nabla_{\max})\sum_{i=1}^{t}(1-{\eta\mu})^i 
    \end{align}
    Since, $\sum_{j=0}^k(1-{\eta\mu} {})^j\leq\frac{1}{\eta\mu}$, for a constant learning rate $\eta$ 
    \begin{align}
        \mathcal{L}(w_{t+1}) \leq (1-{\eta\mu} {})^{t+1} \mathcal{L}(w_0) - \frac{1}{2\mu}(\varepsilon^2-2\varepsilon \nabla_{\max})
    \end{align}    
    We continue to find the ball for which we have convergence, following the difference of weights from \cite{liu2020toward}.
    
    
    \begin{align}
    \left\|w_{t+1}-w_{0}\right\| &=
    \eta\left\|\sum_{\tau=0}^{t} \mathbf{g_{\tau}}\right\| \\
    &\leq \eta \sum_{\tau=0}^{t}\left\|\mathbf{g_{\tau}}\right\|
    \end{align}
    
    Solving (49) for $\|\mathbf{g}_t\| $ we have,$
    % \frac{\eta}{2} \left\|\nabla L_{S}\left(w_{\tau}\right)\right\|^2 &\leq \frac{\beta^2}{\alpha}(\Lc(w_{t})  - \Lc(w_{t+1}) + \frac{\eta \alpha^2}{\beta}\epsilon  \nabla_{\max} - \frac{\eta \alpha^2}{2} \epsilon)
     \left\| \mathbf{g}_t\right\|\leq & \frac{\beta}{\alpha} \sqrt{\frac{2}{\eta}}\sqrt{\Lc(w_{t})  - \Lc(w_{t+1}) + \frac{\eta \alpha^2}{\beta}\epsilon  \nabla_{\max} - \frac{\eta \alpha^2}{2} \epsilon}$
     
     For which we then substitute and continue, 
    \begin{align}
    % &\leq \eta   \sum_{\tau=0}^{t} \frac{\beta}{\alpha} \sqrt{\frac{2}{\eta}}\sqrt{\Lc(w_{t})  - \Lc(w_{t+1}) + \frac{\eta \alpha^2}{\beta}\epsilon  \nabla_{\max} - \frac{\eta \alpha^2}{2} \epsilon}\\
    \left\|w_{t+1}-w_{0}\right\| &\leq 
    \eta \frac{\beta}{\alpha} \sqrt{\frac{2}{\eta}} \sum_{\tau=0}^{t} \sqrt{\Lc(w_{\tau})  - \Lc(w_{\tau+1}) + \frac{\eta \alpha^2}{\beta}\epsilon  \nabla_{\max} - \frac{\eta \alpha^2}{2} \epsilon } \\
    &\leq   \eta \frac{\beta}{\alpha} \sqrt{\frac{2}{\eta}} \sum_{\tau=0}^{t} \sqrt{\Lc(w_{\tau})  + \frac{\eta \alpha^2}{\beta}\epsilon  \nabla_{\max} - \frac{\eta \alpha^2}{2} \epsilon }
    % \end{align}
    % [Note: we might not need to drop $- \frac{\eta \alpha^2}{2} \epsilon$]\\
    % From here we can go two ways. Using (21) first we have 
    % \begin{align}
    % \leq \eta \frac{\beta}{\alpha} \sqrt{\frac{2}{\eta}} \left(\sum_{\tau=0}^{t}(1-\eta \mu)^{\tau / 2}\right) \sqrt{\Lc(w_{0})  + \frac{\eta \alpha^2}{\beta}\epsilon  \nabla_{\max} } \\
    % \leq \eta \frac{\beta}{\alpha} \sqrt{\frac{2}{\eta}}  \sqrt{\Lc(w_{0})  + \frac{\eta \alpha^2}{\beta}\epsilon  \nabla_{\max} } \frac{1}{1-\sqrt{1-\eta \mu}} \\
    % \leq \frac{\beta}{\alpha} \sqrt{\frac{2}{\eta}} \frac{2 \sqrt{\Lc(w_{0})  + \frac{\eta \alpha^2}{\beta}\epsilon  \nabla_{\max} }}{\mu} \\
    % =R
    % \end{align}
    \end{align}
    \text{using Eq. (\ref{eq:adacore_convergence}) we have }\\
    \begin{align}
        &\leq \eta \frac{\beta}{\alpha} \sqrt{\frac{2}{\eta}} \left(\sum_{\tau=0}^{t}(1-\frac{\eta \mu \alpha^2}{\beta^2})^{\tau / 2}\right)\sqrt{\Lc(w_{0})  - \frac{1}{2\mu}(\beta^2\epsilon^2-2\beta\epsilon \nabla_{\max})  + \frac{\eta \alpha^2}{\beta}\epsilon  \nabla_{\max} - \frac{\eta \alpha^2}{2} \epsilon } \\
        &\leq \eta \frac{\beta}{\alpha} \sqrt{\frac{2}{\eta}}  \sqrt{\Lc(w_{0})  - \frac{\beta^2 \epsilon^2}{2\mu} - \frac{\eta \alpha^2}{2} \epsilon + (\frac{\beta}{\mu} + \frac{\alpha^2 \eta}{\beta^2})\epsilon \nabla_{\max} } \frac{1}{1-\sqrt{1-\frac{\eta \mu \alpha^2}{\beta^2}}} \\
    % \leq \frac{\beta}{\alpha} \sqrt{\frac{2}{\eta}} \frac{2 \sqrt{\Lc(w_{0})  + \frac{\eta \alpha^2}{\beta}\epsilon  \nabla_{\max} }}{\mu} \\
    &\leq \frac{2 \beta^3}{ \mu \alpha^3 } \sqrt{\frac{2}{\eta}}  \sqrt{\Lc(w_{0})  - \frac{\beta^2 \epsilon^2}{2\mu} - \frac{\eta \alpha^2}{2} \epsilon + (\frac{\beta}{\mu} + \frac{\alpha^2 \eta}{\beta^2})\epsilon \nabla_{\max} } \\
    &=R
    \end{align}
    
    Thus, $w_{t+1}$ resides in the ball $B(w_o,R)$.
\end{proof}
